Learning-to-Optimize with PAC-Bayesian Guarantees: Theoretical Considerations and Practical Implementation

We use the PAC-Bayesian theory for the setting of learning-to-optimize. To the best of our knowledge, we present the first framework to learn optimization algorithms with provable generalization guarantees (PAC-Bayesian bounds) and explicit trade-off between convergence guarantees and convergence speed, which contrasts with the typical worst-case analysis. Our learned optimization algorithms provably outperform related ones derived from a (deterministic) worst-case analysis. The results rely on PAC-Bayesian bounds for general, possibly unbounded loss-functions based on exponential families. Then, we reformulate the learning procedure into a one-dimensional minimization problem and study the possibility to find a global minimum. Furthermore, we provide a concrete algorithmic realization of the framework and new methodologies for learning-to-optimize, and we conduct four practically relevant experiments to support our theory. With this, we showcase that the provided learning framework yields optimization algorithms that provably outperform the state-of-the-art by orders of magnitude.

==> Experiments/Image_Processing/image_processing_figure_algorithm.tex <==

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}
        \tikzset{conv/.style={black,draw=black,fill=test_1,rectangle,minimum height=0.5cm}}
        \tikzset{linear/.style={black,draw=black,fill=test_2,rectangle,minimum height=0.5cm}}
        \tikzset{relu/.style={black,draw=black,fill=test_3,rectangle,minimum height=0.25cm}}

        % Directions
        \node (d1) at (0, 1.0) {\tiny{$\iter{d}{k}_1$}};
        \node (d2) at (0, 0.0) {\tiny{$\iter{d}{k}_2$}};
        \node (d3) at (-0.4, -1.0) {\tiny{$\iter{d}{k}_1 \odot \iter{d}{k}_2$}};

        % Update Block
        \node[conv,rotate=90,minimum width=2.75cm] (conv1) at (2,0) {\tiny{\texttt{Conv2d(3,16,3,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu1) at (2.5,0) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.75cm] (conv2) at (3,0) {\tiny{\texttt{Conv2d(16,16,3,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2) at (3.5,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv3) at (4,0) {\tiny{\texttt{Conv2d(16,1,3,bias=F)}}};

        \node (d) at (6, 0) {\tiny{$\iter{d}{k}$}};

        \draw[->] (d1) to [out=0, in=180] (conv1.north);
        \draw[->] (d2) to [out=0, in=180] (conv1.north);
        \draw[->] (d3) to [out=0, in=180] (conv1.north);

        \draw[-] (conv1) -- (relu1) -- (conv2) -- (relu2) -- (conv3);
        \draw[->] (conv3) -- (d);

        % Norms
        \node (n1) at (0, -1.9) {\tiny{$\iter{n}{k}_1$}};
        \node (n2) at (0, -3.2) {\tiny{$\iter{n}{k}_2$}};

        % Step-size block
        \node[linear,rotate=90,minimum width=2.3cm] (lin1) at (2, -2.6) {\tiny{\texttt{Linear(2,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_1) at (2.5, -2.6) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin2) at (3, -2.6) {\tiny{\texttt{Linear(8,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_2) at (3.5, -2.6) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin3) at (4, -2.6) {\tiny{\texttt{Linear(8,1,bias=F)}}};

        \node (s) at (6, -2.6) {\tiny{$\iter{s}{k}$}};

        \draw[->] (n1) to [out=0, in=180] (lin1.north);
        \draw[->] (n2) to [out=0, in=180] (lin1.north);

        \draw[-] (lin1) -- (relu2_1) -- (lin2) -- (relu2_2) -- (lin3);
        \draw[->] (lin3) -- (s);

        % Combine to new point
        \node (xk) at (8, 0) {\tiny{$\iter{x}{k}$}};
        \node (new) at (8, -1.3) {\tiny{$\iter{x}{k+1} := \iter{x}{k} + \iter{s}{k} \cdot \iter{d}{k}$}};
        \draw[->] (d) to [out=0, in=90] (new.north);
        \draw[->] (xk) -- (new);
        \draw[->] (s) to [out=0, in=270] (new.south);
        
    \end{tikzpicture}
    \caption{\old{Update step of $\mathcal{A}$ for the image-processing problems: The directions $\iter{d}{k}_1$, $\iter{d}{k}_2$ and $\iter{d}{k}_1 \odot \iter{d}{k}_2$ are inserted as different channels (in the shape of the image) into the \texttt{Conv2d}-block, which performs a $3 \times 3$-convolution. The scales $\iter{n}{1}$, $\iter{n}{2}$ get transformed separately by the fully-connected block.}}
    \label{architecture:image_processing}
\end{figure}

==> Experiments/Lasso/lasso_figure_algorithm.tex <==

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}

        \tikzset{conv/.style={black,draw=black,fill=test_1,rectangle,minimum height=0.5cm}}
        \tikzset{linear/.style={black,draw=black,fill=test_2,rectangle,minimum height=0.5cm}}
        \tikzset{relu/.style={black,draw=black,fill=test_3,rectangle,minimum height=0.25cm}}
        \tikzset{sigmoid/.style={black,draw=black,fill=test_4,rectangle,minimum height=0.25cm}}
        
        % Directions
        \node (d1) at (0, -0.9) {\tiny{$\iter{d}{k}_1$}};
        \node (d2) at (0, -0.3) {\tiny{$\iter{d}{k}_2$}};
        \node (d3) at (-0.4, 0.3) {\tiny{$\iter{d}{k}_1 \odot \iter{d}{k}_2$}};
        \node (d4) at (0, 0.9) {\tiny{$\iter{d}{k}_3$}};

        % Update Block
        \node[conv,rotate=90,minimum width=2.75cm] (conv1) at (1.4, 0) {\tiny{\texttt{Conv2d(4,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu1) at (1.9, 0) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.75cm] (conv2) at (2.4, 0) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2) at (2.9, 0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv3) at (3.4, 0) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu3) at (3.9, 0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv4) at (4.4, 0) {\tiny{\texttt{Conv2d(64,1,1,bias=F)}}};

        \node (d) at (5.3, 0) {\tiny{$\iter{d}{k}$}};

        \draw[->] (d1) to [out=0, in=180] (conv1.north);
        \draw[->] (d2) to [out=0, in=180] (conv1.north);
        \draw[->] (d3) to [out=0, in=180] (conv1.north);
        \draw[->] (d4) to [out=0, in=180] (conv1.north);

        \draw[-] (conv1) -- (relu1) -- (conv2) -- (relu2) -- (conv3) -- (relu3) -- (conv4);
        \draw[->] (conv4) -- (d);

        % Norms
        \node (n1) at (0, -2.1) {\tiny{$\iter{n}{k}_1$}};
        \node (n2) at (0, -2.7) {\tiny{$\iter{n}{k}_2$}};
        \node (n3) at (0, -3.3) {\tiny{$\iter{n}{k}_3$}};

        % Step-size block
        \node[linear,rotate=90,minimum width=2.5cm] (lin1) at (1.4, -2.7) {\tiny{\texttt{Linear(3,64,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.5cm] (relu2_1) at (1.9, -2.7) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.5cm] (lin2) at (2.4, -2.7) {\tiny{\texttt{Linear(64,64,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.5cm] (relu2_2) at (2.9, -2.7) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.5cm] (lin3) at (3.4, -2.7) {\tiny{\texttt{Linear(64,64,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.5cm] (relu2_3) at (3.9, -2.7) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.5cm] (lin4) at (4.4, -2.7) {\tiny{\texttt{Linear(64,1,bias=F)}}};

        \node (s) at (5.3, -2.7) {\tiny{$\iter{s}{k}$}};

        \draw[->] (n1) to [out=0, in=180] (lin1.north);
        \draw[->] (n2) to [out=0, in=180] (lin1.north);
        \draw[->] (n3) to [out=0, in=180] (lin1.north);

        \draw[-] (lin1) -- (relu2_1) -- (lin2) -- (relu2_2) -- (lin3) -- (relu2_3) -- (lin4);
        \draw[->] (lin4) -- (s);

        % Combine to new point
        \node (new) at (5.9, -1.35) {\tiny{$\iter{\Tilde{x}}{k+1}$}};
        \node (xk) at (5.9, -3.5) {\tiny{$\iter{x}{k}$}};
        \draw[->] (xk) -- (new);
        \draw[->] (d) to [out=270, in=90] (new.north);
        \draw[->] (s) to [out=90, in=270] (new.south);

        % Sparsity Block
        \node[conv,rotate=90,minimum width=2.75cm] (conv2_1) at (7.,-1.35) {\tiny{\texttt{Conv2d(3,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2_1) at (7.5,-1.35) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.75cm] (conv2_2) at (8.,-1.35) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2_2) at (8.5,-1.35) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv2_3) at (9.,-1.35) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2_3) at (9.5,-1.35) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv2_4) at (10.,-1.35) {\tiny{\texttt{Conv2d(64,1,1,bias=F)}}};
        \node[sigmoid,rotate=90,minimum width=2.75cm] (sig) at (10.5,-1.35) {\tiny{\texttt{Sigmoid}}};

        \draw[->] (new) -- (conv2_1);
        \draw[->] (xk) to [out=0,in=270] (conv2_1.west);
        \draw[->] (d4) to [out=90,in=90] (conv2_1.east);

        \node (sp) at (11.2, -1.35) {\tiny{$z$}};
        \draw[-] (conv2_1) -- (relu2_1) -- (conv2_2) -- (relu2_2) -- (conv2_3) -- (relu2_3) -- (conv2_4) -- (sig);
        \draw[->] (sig) -- (sp);

        \draw (12, -2.35) circle [radius=0.25] node (tau) {\tiny{$\tau$}};
        \node (next) at (13, -1.35) {\tiny{$\text{prox}_\tau(z \odot \iter{\Tilde{x}}{k+1})$}};
        \draw[->] (sp) -- (next);
        \draw[->] (new) to [out=90,in=90] (next.north);
        \draw[->] (tau) -- (next);
        
    \end{tikzpicture}
    \caption{\old{Algorithmic update for the Lasso-problem: Additionally to the directions $\iter{d}{k}_1$, $\iter{d}{k}_2$ and $\iter{d}{k}_1 \odot \iter{d}{k}_2$, we add the subgradient $\partial \norm{\iter{x}{k}}{1}$ as input $\iter{d}{k}_3$. Hence, also the lower block, which computes the step-size $\iter{s}{k}$, gets an additional input $\iter{n}{k}_3$, namely the (transformed) norm of the subgradient. Then, $\iter{d}{k}$ and $\iter{s}{k}$ get used to compute a new point $\iter{\Tilde{x}}{k+1} := \iter{x}{k} + \iter{s}{k} \cdot \iter{d}{k}$, which, together with the current point $\iter{x}{k}$ and the subgradient, gets fed into the \say{sparsity-block}, which computes a vector in $[0,1]^d$ that is used to decrease the coordinates of $\iter{\Tilde{x}}{k+1}$. Finally, we apply the proximal-map with learned parameter $\tau$ to get the next iterate.}}
    \label{architecture:lasso}
\end{figure}

==> Experiments/Lasso/lasso_figure_algorithm_test.tex <==

    \begin{tikzpicture}

        \tikzset{conv/.style={black,draw=black,fill=test_1,rectangle,minimum height=0.5cm}}
        \tikzset{linear/.style={black,draw=black,fill=test_2,rectangle,minimum height=0.5cm}}
        \tikzset{relu/.style={black,draw=black,fill=test_3,rectangle,minimum height=0.25cm}}
        \tikzset{sigmoid/.style={black,draw=black,fill=test_4,rectangle,minimum height=0.25cm}}
        
        % Directions
        \node (d1) at (0, -0.9) {\tiny{$\iter{d}{k}_1$}};
        \node (d2) at (0, -0.3) {\tiny{$\iter{d}{k}_2$}};
        \node (d3) at (-0.4, 0.3) {\tiny{$\iter{d}{k}_1 \odot \iter{d}{k}_2$}};
        \node (d4) at (0, 0.9) {\tiny{$\iter{d}{k}_3$}};

        % Update Block
        \node[conv,rotate=90,minimum width=2.75cm] (conv1) at (1.4, 0) {\tiny{\texttt{Conv2d(4,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu1) at (1.9, 0) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.75cm] (conv2) at (2.4, 0) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2) at (2.9, 0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv3) at (3.4, 0) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu3) at (3.9, 0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv4) at (4.4, 0) {\tiny{\texttt{Conv2d(64,1,1,bias=F)}}};

        \node (d) at (5.3, 0) {\tiny{$\iter{d}{k}$}};

        \draw[->] (d1) to [out=0, in=180] (conv1.north);
        \draw[->] (d2) to [out=0, in=180] (conv1.north);
        \draw[->] (d3) to [out=0, in=180] (conv1.north);
        \draw[->] (d4) to [out=0, in=180] (conv1.north);

        \draw[-] (conv1) -- (relu1) -- (conv2) -- (relu2) -- (conv3) -- (relu3) -- (conv4);
        \draw[->] (conv4) -- (d);

        % Norms
        \node (n1) at (0, -2.1) {\tiny{$\iter{n}{k}_1$}};
        \node (n2) at (0, -2.7) {\tiny{$\iter{n}{k}_2$}};
        \node (n3) at (0, -3.3) {\tiny{$\iter{n}{k}_3$}};

        % Step-size block
        \node[linear,rotate=90,minimum width=2.5cm] (lin1) at (1.4, -2.7) {\tiny{\texttt{Linear(3,64,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.5cm] (relu2_1) at (1.9, -2.7) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.5cm] (lin2) at (2.4, -2.7) {\tiny{\texttt{Linear(64,64,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.5cm] (relu2_2) at (2.9, -2.7) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.5cm] (lin3) at (3.4, -2.7) {\tiny{\texttt{Linear(64,64,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.5cm] (relu2_3) at (3.9, -2.7) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.5cm] (lin4) at (4.4, -2.7) {\tiny{\texttt{Linear(64,1,bias=F)}}};

        \node (s) at (5.3, -2.7) {\tiny{$\iter{s}{k}$}};

        \draw[->] (n1) to [out=0, in=180] (lin1.north);
        \draw[->] (n2) to [out=0, in=180] (lin1.north);
        \draw[->] (n3) to [out=0, in=180] (lin1.north);

        \draw[-] (lin1) -- (relu2_1) -- (lin2) -- (relu2_2) -- (lin3) -- (relu2_3) -- (lin4);
        \draw[->] (lin4) -- (s);

        % Combine to new point
        \node (new) at (5.9, -1.35) {\tiny{$\iter{\Tilde{x}}{k+1}$}};
        \node (xk) at (5.9, -3.5) {\tiny{$\iter{x}{k}$}};
        \draw[->] (xk) -- (new);
        \draw[->] (d) to [out=270, in=90] (new.north);
        \draw[->] (s) to [out=90, in=270] (new.south);

        % Sparsity Block
        \node[conv,rotate=90,minimum width=2.75cm] (conv2_1) at (7.,-1.35) {\tiny{\texttt{Conv2d(3,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2_1) at (7.5,-1.35) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.75cm] (conv2_2) at (8.,-1.35) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2_2) at (8.5,-1.35) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv2_3) at (9.,-1.35) {\tiny{\texttt{Conv2d(64,64,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2_3) at (9.5,-1.35) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv2_4) at (10.,-1.35) {\tiny{\texttt{Conv2d(64,1,1,bias=F)}}};
        \node[sigmoid,rotate=90,minimum width=2.75cm] (sig) at (10.5,-1.35) {\tiny{\texttt{Sigmoid}}};

        \draw[->] (new) -- (conv2_1);
        \draw[->] (xk) to [out=0,in=270] (conv2_1.west);
        \draw[->] (d4) to [out=90,in=90] (conv2_1.east);

        \node (sp) at (11.2, -1.35) {\tiny{$z$}};
        \draw[-] (conv2_1) -- (relu2_1) -- (conv2_2) -- (relu2_2) -- (conv2_3) -- (relu2_3) -- (conv2_4) -- (sig);
        \draw[->] (sig) -- (sp);

        \draw (12, -2.35) circle [radius=0.25] node (tau) {\tiny{$\tau$}};
        \node (next) at (13, -1.35) {\tiny{$\text{prox}_\tau(z \odot \iter{\Tilde{x}}{k+1})$}};
        \draw[->] (sp) -- (next);
        \draw[->] (new) to [out=90,in=90] (next.north);
        \draw[->] (tau) -- (next);
        
    \end{tikzpicture}



==> Experiments/Neural_Network_Training/neural_network_figure_algorithm.tex <==

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}
        \tikzset{conv/.style={black,draw=black,fill=test_1,rectangle,minimum height=0.5cm}}
        \tikzset{linear/.style={black,draw=black,fill=test_2,rectangle,minimum height=0.5cm}}
        \tikzset{relu/.style={black,draw=black,fill=test_3,rectangle,minimum height=0.25cm}}

        % Norms
        \node (n1) at (-4, 1.8) {\tiny{$\iter{n}{k}_1$}};
        \node (n2) at (-4, 0.9) {\tiny{$\iter{n}{k}_2$}};
        \node (l1) at (-4, 0) {\tiny{$\iter{\ell}{k}$}};
        \node (l2) at (-4, -0.9) {\tiny{$\iter{\ell}{k-1}$}};
        \node (s) at (-4, -1.8) {\tiny{$\iter{s}{k}$}};

        % Step-size block
        \node[linear,rotate=90,minimum width=2.3cm] (lin1) at (-3, 0) {\tiny{\texttt{Linear(5,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_1) at (-2.5, 0) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin2) at (-2.0, 0) {\tiny{\texttt{Linear(8,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_2) at (-1.5, 0) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin3) at (-1.0, 0) {\tiny{\texttt{Linear(8,4,bias=F)}}};

        \draw[->] (n1) to [out=0, in=180] (lin1.north);
        \draw[->] (n2) to [out=270, in=180] (lin1.north);
        \draw[->] (l1) to [out=0, in=180] (lin1.north);
        \draw[->] (l2) to [out=90, in=180] (lin1.north);
        \draw[->] (s) to [out=0, in=180] (lin1.north);

        \node (s1) at (0.1, 1.25) {\tiny{$s_1$}};
        \node (s2) at (0.1, 0.325) {\tiny{$s_2$}};
        \node (s3) at (0.1, -0.325) {\tiny{$s_3$}};
        \node (s4) at (0.1, -1.25) {\tiny{$s_4$}};

        \draw[->] (lin3.south) to [out=0, in=180] (s1.west);
        \draw[->] (lin3.south) to [out=0, in=180] (s2.west);
        \draw[->] (lin3.south) to [out=0, in=180] (s3.west);
        \draw[->] (lin3.south) to [out=0, in=180] (s4.west);

        \draw[-] (lin1) -- (relu2_1) -- (lin2) -- (relu2_2) -- (lin3);

        % Directions
        \draw (1, 2.) circle [radius=0.18] node (g) {\tiny{$g$}};
        \draw (1, -2.) circle [radius=0.18] node (m) {\tiny{$m$}};
        \node (d1) at (1.5, 1.25) {\tiny{$s_1 \cdot g \odot \iter{d}{k}_1$}};
        \node (d2) at (1.8, 0.325) {\tiny{$s_2 \cdot \iter{d}{k}_1$}};
        \node (d3) at (1.8, -0.325) {\tiny{$s_3 \cdot \iter{d}{k}_2$}};
        \node (d4) at (1.5, -1.25) {\tiny{$s_4 \cdot m \odot \iter{d}{k}_2$}};
        
        \node (xk) at (2.5, 2.) {\tiny{$\iter{x}{k}$}};
        \node (xkm1) at (2.5, -2.) {\tiny{$\iter{x}{k-1}$}};

        \draw[->] (g) to [out=0,in=90] (d1.north);
        \draw[->] (s1) to (d1.west);
        \draw[->] (s2) to (d2.west);
        \draw[->] (s3) to (d3.west);
        \draw[->] (s4) to (d4.west);
        \draw[->] (m) to [out=0, in=270] (d4.south);

        % Update Block
        \node[conv,rotate=90,minimum width=2.7cm] (conv1) at (3.25,0) {\tiny{\texttt{Conv2d(6,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.7cm] (relu1) at (3.75,0) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.7cm] (conv2) at (4.25,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.7cm] (relu2) at (4.75,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.7cm] (conv3) at (5.25,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.7cm] (relu3) at (5.75,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.7cm] (conv4) at (6.25,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.7cm] (relu4) at (6.75,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.7cm] (conv5) at (7.25,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.7cm] (relu5) at (7.75,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.7cm] (conv6) at (8.25,0) {\tiny{\texttt{Conv2d(16,1,1,bias=F)}}};

        \node (d) at (9.2, 0) {\tiny{$\iter{d}{k}$}};

        \draw[->] (xk) to [out=0,in=90] (conv1.east);
        \draw[->] (xkm1) to [out=0,in=270] (conv1.west);
        
        \draw[->] (d1) to [out=0, in=180] (conv1.north);
        \draw[->] (d2) to [out=0, in=180] (conv1.north);
        \draw[->] (d3) to [out=0, in=180] (conv1.north);
        \draw[->] (d4) to [out=0, in=180] (conv1.north);

        \draw[-] (conv1) -- (relu1) -- (conv2) -- (relu2) -- (conv3) -- (relu3) -- (conv4) -- (relu4) -- (conv5) -- (relu5) -- (conv6);
        \draw[->] (conv6) -- (d);

        % Combine to new point
        \node (new) at (10.4, 0) {\tiny{$\iter{x}{k+1}$}};
        \draw[->] (xk) to [out=0, in=90] (new.north);
        \draw[->] (d) -- (new);
        
    \end{tikzpicture}
    \caption{\old{Algorithmic update for training the neural network: Based on the two norms $\iter{n}{k}_1$ and $\iter{n}{k}_2$, the scalar product $\iter{s}{k} := \sprod{\iter{d}{k}_1}{\iter{d}{k}_2}$, and the current and previous (logarithmically scaled) loss $\iter{\ell}{k}$, $\iter{\ell}{k-1}$, we compute four scalars $s_1, ..., s_4$, which are used for weighting $\iter{d}{k}_1$, $\iter{d}{k}_2$, and their corresponding pre-conditioned versions $g \odot \iter{d}{k}_1$ and $m \odot \iter{d}{k}_2$. Together with the current and previous point, they get fed (as separate channels) into the first layer of a 1x1-convolutional block, which computes an update direction $\iter{d}{k}$. Then, we update $\iter{x}{k+1} := \iter{x}{k} + \iter{d}{k}$.}}
    \label{architecture:neural_network}
\end{figure}

==> Experiments/Quadratics/quadratics_figure_algorithm.tex <==

\begin{figure}[t!]
    \centering
    \begin{tikzpicture}
        \tikzset{conv/.style={black,draw=black,fill=test_1,rectangle,minimum height=0.5cm}}
        \tikzset{linear/.style={black,draw=black,fill=test_2,rectangle,minimum height=0.5cm}}
        \tikzset{relu/.style={black,draw=black,fill=test_3,rectangle,minimum height=0.25cm}}

        % Directions
        \node (d1) at (0, 1.0) {\tiny{$\iter{d}{k}_1$}};
        \node (d2) at (0, 0.0) {\tiny{$\iter{d}{k}_2$}};
        \node (d3) at (-0.4, -1.0) {\tiny{$\iter{d}{k}_1 \odot \iter{d}{k}_2$}};

        % Update Block
        \node[conv,rotate=90,minimum width=2.75cm] (conv1) at (2,0) {\tiny{\texttt{Conv2d(3,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu1) at (2.5,0) {\tiny{\texttt{ReLU}}};
        
        \node[conv,rotate=90,minimum width=2.75cm] (conv2) at (3,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[conv,rotate=90,minimum width=2.75cm] (conv3) at (3.5,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu2) at (4,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv4) at (4.5,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[conv,rotate=90,minimum width=2.75cm] (conv5) at (5,0) {\tiny{\texttt{Conv2d(16,16,1,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.75cm] (relu3) at (5.5,0) {\tiny{\texttt{ReLU}}};

        \node[conv,rotate=90,minimum width=2.75cm] (conv6) at (6,0) {\tiny{\texttt{Conv2d(16,1,1,bias=F)}}};

        \node (d) at (7, 0) {\tiny{$\iter{d}{k}$}};

        \draw[->] (d1) to [out=0, in=180] (conv1.north);
        \draw[->] (d2) -- (conv1);
        \draw[->] (d3) to [out=0, in=180] (conv1.north);

        \draw[-] (conv1) -- (relu1) -- (conv2) -- (conv3) -- (relu2) -- (conv4) -- (conv5) -- (relu3) -- (conv6);
        \draw[->] (conv6) -- (d);

        % Norms
        \node (n1) at (0, -2.) {\tiny{$\iter{n}{k}_1$}};
        \node (n2) at (0, -3.2) {\tiny{$\iter{n}{k}_2$}};

        % Step-size block
        \node[linear,rotate=90,minimum width=2.3cm] (lin1) at (2, -2.6) {\tiny{\texttt{Linear(2,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_1) at (2.5, -2.6) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin2) at (3, -2.6) {\tiny{\texttt{Linear(8,8,bias=F)}}};
        \node[linear,rotate=90,minimum width=2.3cm] (lin3) at (3.5, -2.6) {\tiny{\texttt{Linear(8,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_2) at (4.0, -2.6) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin4) at (4.5, -2.6) {\tiny{\texttt{Linear(8,8,bias=F)}}};
        \node[linear,rotate=90,minimum width=2.3cm] (lin5) at (5.0, -2.6) {\tiny{\texttt{Linear(8,8,bias=F)}}};
        \node[relu,rotate=90,minimum width=2.3cm] (relu2_3) at (5.5, -2.6) {\tiny{\texttt{ReLU}}};

        \node[linear,rotate=90,minimum width=2.3cm] (lin6) at (6, -2.6) {\tiny{\texttt{Linear(8,1,bias=F)}}};

        \node (s) at (7, -2.6) {\tiny{$\iter{s}{k}$}};

        \draw[->] (n1) to [out=0, in=180] (lin1.north);
        \draw[->] (n2) to [out=0, in=180] (lin1.north);

        \draw[-] (lin1) -- (relu2_1) -- (lin2) -- (lin3) -- (relu2_2) -- (lin4) -- (lin5) -- (relu2_3) -- (lin6);
        \draw[->] (lin6) -- (s);

        % Combine to new point
        \node (xk) at (9, 0) {\tiny{$\iter{x}{k}$}};
        \node (new) at (9, -1.3) {\tiny{$\iter{x}{k+1} := \iter{x}{k} + \iter{s}{k} \cdot \iter{d}{k}$}};
        \draw[->] (d) to [out=0, in=90] (new.north);
        \draw[->] (xk) -- (new);
        \draw[->] (s) to [out=0, in=270] (new.south);
        
    \end{tikzpicture}
    \caption{\old{Update step of $\mathcal{A}$ for quadratic problems: The directions $\iter{d}{k}_1$, $\iter{d}{k}_2$ and $\iter{d}{k}_1 \odot \iter{d}{k}_2$ are inserted as different channels into the \texttt{Conv2d}-block, which performs $1 \times 1$ \say{convolutions}, that is, the algorithm acts coordinate-wise on the input. The scales $\iter{n}{1}$, $\iter{n}{2}$ get transformed separately by the fully-connected block.}}
    \label{architecture:quadratics}
\end{figure}

==> Supplementary_Material.tex <==

\subsection{On the Finiteness Assumption of $\Lambda$} 

We denote the open ball of radius $r$ around a point $x$ by $\mathcal{B}(x; r)$ and the corresponding closed ball by $\mathcal{B}[x; r]$. For a set $S$, the notation $\vert S \vert$ denotes the cardinality of $S$.

\begin{Def}[Totally Bounded Space]
    A metric space $(\space{X}, d)$ is called \emph{totally bounded}, if for every $\epsilon > 0$ there exists $n \in \mathbb{N}$, $x_1,...,x_n \in \space{X}$, such that
    $$
        \space{X} \subseteq \bigcup_{i=1}^n \mathcal{B}(x_i;\epsilon) \,.
    $$
\end{Def}

The typical example of a totally bounded space is a compact space. The important property of this space, which is used in the following, is that they have a finite covering number. In the end, this allows again to apply the union bound argument.

\begin{Def}[$\delta$-Covering Number]
    Let $(\space{X}, d)$ be a totally bounded metric space and let $\delta > 0$. A \emph{proper $\delta$-covering} of $\space{X}$ is a finite set $X_\delta \subset \space{X}$, such that
    $$
        \space{X} \subseteq \bigcup_{x \in X_\delta} \mathcal{B}[x;\delta] \,.
    $$
    The minimal cardinality of any $\delta$-covering is denoted $\coveringNumber{\delta}{\space{X}}$ and is called the \emph{$\delta$-covering number} of $\space{X}$:
    $$
        \coveringNumber{\delta}{\space{X}} := \min \{\vert X_\delta \vert \ : \ \text{$X_\delta$ is a proper $\delta$-covering of $\space{X}$}\} \,.
    $$
\end{Def}

Taken together, and using the proof of Theorem \ref{Thm_PACBayes_exponential_familiy} as entry point, one gets the following Lemma. This is a direct generalization of the result in Theorem \ref{Thm_PACBayes_exponential_familiy}, as in the case where $\Lambda$ is finite, $\Lambda$ can be covered by itself, such that it holds $\coveringNumber{\delta}{\Lambda} = \vert \Lambda \vert$ and $C = 0$.

\begin{Lem}\label{proof_LambdaFiniteNotNecessary}
    Let $(\Lambda, d)$ be a totally bounded metric space and let $\delta > 0$. Assume that there is a constant $C(\delta)$, such that for all $\Tilde{\lambda} \in \Lambda$ and $d \in \space{D}_N$ it holds: 
    $$
    \sup_{\lambda \in \closedBall{\Tilde{\lambda}}{\delta}} \kappa_d(\lambda) - \kappa_d(\Tilde{\lambda}) \le C(\delta) \,.
    $$
    Finally, assume that $\mathbb{P} \{ \kappa(\lambda, \rvec{D}_N) > s  \} \le \exp(-s)$ for all $s \in \mathbb{R}$, $\lambda \in \Lambda$. Then it holds that:
    $$
        \mathbb{P} \Bigl\{ \sup_{\lambda \in \Lambda} \kappa(\lambda, \rvec{D}_N) \le \log \Bigl( \frac{\coveringNumber{\delta}{\Lambda}}{\epsilon} \Bigr) + C(\delta) \Bigr\} \ge 1-\epsilon \,.
    $$
\end{Lem}
\begin{proof}
    Since $(\Lambda, d)$ is a totally bounded metric space, its covering number $\coveringNumber{\delta}{\Lambda}$ is well-defined and finite. For notational simplicity, set $N := \coveringNumber{\delta}{\Lambda}$. Hence, there are $\lambda_1, ..., \lambda_N \in \Lambda$, such that:
    $$
        \Lambda \subseteq \bigcup_{i=1}^N \closedBall{\lambda_i}{\delta} \,.
    $$
    Therefore, one directly gets for every $d \in \space{D}_N$:
    $$
        \sup_{\lambda \in \Lambda} \kappa_d(\lambda) \le \max_{i=1,...,N} \ \sup_{\lambda \in \closedBall{\lambda_i}{\delta}} \kappa_d(\lambda) \,.
    $$
    Further, by assumption it holds:
    $$
        \sup_{\lambda \in \closedBall{\lambda_i}{\delta}} \kappa_d(\lambda) 
        = \kappa_d(\lambda_i) + \sup_{\lambda \in \closedBall{\lambda_i}{\delta}} \Bigr(\kappa_d(\lambda) - \kappa_d(\lambda_i) \Bigl) 
        \le \kappa_d(\lambda_i) + C(\delta) \,.
    $$
    Hence, in total one gets for $s \in \mathbb{R}$:
    \begin{align*}
        \prob \left\{ \sup_{\lambda \in \Lambda} \kappa(\lambda, \rvec{D}_N) > s \right\} 
        &\le \prob \left\{ \max_{i=1,...,N} \kappa(\lambda_i, \rvec{D}_N) + C(\delta) > s \right\}  \\
        &= \prob \bigcup_{i=1}^N \{\kappa(\lambda_i, \rvec{D}_N) + C(\delta) > s\} \\
        &\le \sum_{i=1}^N \prob \left\{ \kappa(\lambda_i, \rvec{D}_N) + C(\delta) > s \right\} \\
        &\le \sum_{i=1}^N \exp(C(\delta)-s) \\
        &= N \exp(C(\delta)-s) \,.
    \end{align*}
    Since $\epsilon = N \exp(C-s) \ \iff s = \log\left( \frac{N}{\epsilon} \right) + C(\delta)$, one gets:
    $$
    \mathbb{P} \left\{ \sup_{\lambda \in \Lambda} \kappa(\lambda, \rvec{D}_N) > \log\left( \frac{N}{\epsilon} \right) + C(\delta) \right\} \le \epsilon\,.
    $$
    Taking the complementary event yields the result:
    $$
    \mathbb{P} \left\{ \sup_{\lambda \in \Lambda} \kappa(\lambda, \rvec{D}_N) \le \log\left( \frac{N}{\epsilon} \right) + C(\delta) \right\} \ge 1-\epsilon\,.
    $$
\end{proof}

\begin{Rem}
    One typical example, for which the assumption 
    $$
    \sup_{\lambda \in \closedBall{\Tilde{\lambda}}{\delta}} \kappa_d(\lambda) - \kappa_d(\Tilde{\lambda}) \le C(\delta)
    $$ is verified easily, is the case when $\kappa$ is continuous. In this case, by restricting $\Lambda$ to a compact set, one can take $\kappa$ to be Lipschitz-continuous with some constant $L \ge 0$, which, by definition guarantees the corresponding growth condition with $C(\delta) = L \delta$.
\end{Rem}

